Multiwavelength Spectral Analysis and Neural Network Classification of Counterparts to 4FGL Unassociated Sources

The Fermi-LAT unassociated sources represent some of the most enigmatic gamma-ray sources in the sky. Observations with the Swift-XRT and -UVOT telescopes have identified hundreds of likely X-ray and UV/optical counterparts in the uncertainty ellipses of the unassociated sources. In this work we present spectral fitting results for 205 possible X-ray/UV/optical counterparts to 4FGL unassociated targets. Assuming that the unassociated sources contain mostly pulsars and blazars, we develop a neural network classifier approach that applies gamma-ray, X-ray, and UV/optical spectral parameters to yield descriptive classification of unassociated spectra into pulsars and blazars. From our primary sample of 174 Fermi sources with a single X-ray/UV/optical counterpart, we present 132 P_bzr > 0.99 likely blazars and 14 P_bzr < 0.01 likely pulsars, with 28 remaining ambiguous. These subsets of the unassociated sources suggest a systematic expansion to catalogs of gamma-ray pulsars and blazars. Compared to previous classification approaches our neural network classifier achieves significantly higher validation accuracy and returns more bifurcated P_bzr values, suggesting that multiwavelength analysis is a valuable tool for confident classification of Fermi unassociated sources.

==> tables/XRTMult.tex <==
\startlongtable
\begin{deluxetable*}{cccl}% C for mathmode
\tablecaption{4FGL unassociated sources with more than one notable excess in their error ellipse, along with the numbers of photons counted from each ellipse to quickly compare fluxes. \label{tab:DoubleTroubles}}
\tablewidth{\columnwidth}
\tablehead{
\colhead{4FGL Name} & \colhead{\# XRT notable excesses} & \colhead{Counts} & \colhead{Notes} } 
\startdata
J0126.3$-$6746 & 2 & 84/35 & \\
J0523.3$-$2527 & 2 & 940/209 & \\
J0544.8+5209 & 2 & 32/29 & \\ 
J0610.8$-$4911 & 2 & 369/39 & \\
J0738.6+1311 & 2 & 40/24 & \\
J0800.1$-$5531 & 2 & 32/29 & \\
J1008.2$-$1000 & 3 & 2804/71/31 & \\
J1011.1$-$4420 & 2 & 1598/33 & \\
J1018.1$-$4051 & 2 & 46/44 & \\
J1326.0+3507 & 3 & 77/75/50 & \\
J1637.5+3005 & 3 & 119/59/35 & \\
J1649.2$-$4513 & 4 & 249/437/337/398 & uneven coverage, removed \\
J1808.5$-$3701 & 4 & 83226/790/947/633 & \\
J1836.8$-$2354 & 5 & 647/369/244/365/259 & uneven coverage, removed \\
J1846.9$-$0227 & 2 & 288/180 & \\ 
J1910.8+2856 & 2 & 263/52 & \\
J2351.4$-$2818 & 2 & 67/48 & \\
\enddata
\tablenotetext{}{}
\end{deluxetable*}

==> tables/XRT_star_buddies.tex <==
J1513.0-3118 & -11.50 & 2.37 & 5.51 & 2.11 & \textit{J151244.8-311647} & -11.88 & 3.01 & uu & 15.00 & -0.9998- \\ \hline 
J0738.6+1311 & -11.54 & 2.53 & 10.49 & 0.78 & \textit{J073843.4+131330} & -12.54 & 2.29 & uu & 13.37 & -0.9998- \\ 
J1846.9-0227 & -10.47 & 2.47 & 6.89 & 5.24 & \textit{J184650.7-022904} & -8.97 & 7.90 & uu & 13.96 & -0.9999- \\ 

J1008.2-1000 & -11.43 & 3.14 & 8.92 & 1.10 & J100749.3-094910 & -12.50 & 1.64 & uu & 19.54 & 0.9986 \\ 
 &  &  &  &  & J100802.5-095918 & -11.77 & 1.10 & uu & 19.30 & 0.9989 \\ 
 &  &  &  &  & J100848.6-095450 & -10.78 & 1.88 & uu & 15.16 & 0.9998 \\ \hline 
